Real-Time Toxicity Filtering for Open-Source Code Reviews

Toxic interactions in open-source software development harm community collaboration. To combat this, we propose ToxiShield, a realtime browser extension that identifies and detoxifies toxic code reviews. The framework comprises three modules: toxicity identification, reasoned multiclass classification, and code review detoxification. Our fine-tuned BERT-based binary classifier achieved a 97% F1-score on 38,761 code review texts. For multiclass classification, Claude 3.5 Sonnet with prompt engineering achieved a 39% MCC and 42% F1 on 1,200 samples. Finally, our fine-tuned Llama 3.2 detoxification model reached 95.27% style transfer accuracy, 97.03% fluency, 67.07% content preservation, and an 84% J-score. Validation with 10 software developers suggests ToxiShield effectively fosters a more inclusive open-source environment.

==> Sections/conclusion.tex <==

\section{Conclusion and Future Work}
\label{sec:conclusion}



==> Sections/hypothesis.tex <==
\section{Hypothesis}
\label{sec:hypo}


==> Sections/implication.tex <==

\section{Implications and Future Directions}
\label{sec:impl}


==> Sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}








==> Sections/related_works.tex <==
\section{Background and Related Work}
\label{sec:background}



==> Sections/threats.tex <==
\section{Threats to Validity}
\label{sec:threats}

